SegViT: Semantic Segmentation with Plain Vision Transformers

We explore the capability of plain Vision Transformers (ViTs) for semantic segmentation and propose the SegVit. Previous ViT-based segmentation networks usually learn a pixel-level representation from the output of the ViT. Differently, we make use of the fundamental component -- attention mechanism, to generate masks for semantic segmentation. Specifically, we propose the Attention-to-Mask (ATM) module, in which the similarity maps between a set of learnable class tokens and the spatial feature maps are transferred to the segmentation masks. Experiments show that our proposed SegVit using the ATM module outperforms its counterparts using the plain ViT backbone on the ADE20K dataset and achieves new state-of-the-art performance on COCO-Stuff-10K and PASCAL-Context datasets. Furthermore, to reduce the computational cost of the ViT backbone, we propose query-based down-sampling (QD) and query-based up-sampling (QU) to build a Shrunk structure. With the proposed Shrunk structure, the model can save up to $40\%$ computations while maintaining competitive performance.

==> nips2022 segvit_arXiv/supple.tex <==














\paragraph{}
In this section, we show more evaluation results to demonstrate the performance of the proposed SegViT structure.

\begin{figure}[t]
\raisebox{-1\height}{\vspace{0pt}\includegraphics[width=0.6\textwidth]{figures/supp/supp.pdf}}\hfill%
\begin{minipage}[t]{0.35\textwidth}
\caption{
Accuracy vs.\ computational cost on the ADE20K \texttt{val.}\ split. All the performances and computational costs are measured at single scale inference.  Our proposed SegViT structure can achieve a better trade-off and the best performance among methods using ViT backbone. 
}
 \label{fig:supp}
\end{minipage}
\end{figure}

\subsection{Illustration of the accuracy vs.\ computational cost}
As shown in \cref{fig:supp}, we achieve the best performance with a better trade-off between computational cost and accuracy compared to other methods that use ViT backbone. Also, for our SegViT \emph{Shrunk} version, we dramatically reduced the computation while still retaining competitive performance. 

\subsection{More Visualization Results}

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/supp/ade.pdf}
    \caption{
    Competitive segmentation results on the ADE20K \texttt{val.} split.}
    \label{fig:ade}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/supp/coco.pdf}
    \caption{Competitive segmentation results on the COCO-stuff-10K dataset.}
    \label{fig:coco}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/supp/pc.pdf}
    \caption{Competitive segmentation results on the PASCAL-Context  dataset with $60$ classes.}
    \label{fig:pc}
\end{figure}

\paragraph{Competitive segmentation results on three datasets.}
\cref{fig:ade}, \cref{fig:coco} and \cref{fig:pc} illustrates the model performance on ADE20K, COCO-Stuff-10K and PASCAL-Context datasets respectively using single-scale inference. We can see that in various indoor and outdoor scenes, SegViT can produce satisfactory segmentation results. 








\subsection{More Ablation Study Results}
Different decoder methods have their corresponding feature merge types and loss types. We compare the difference on a plain ViT base backbone shown in Table~\ref{tab:struct compare}. For hierarchical backbones, such as Swin, since the resolution of the feature maps of each stage is reduced, to get feature maps with large resolution and rich semantic information, FPN is necessary. However, in Table~\ref{tab:struct compare}, FPN structure can not work well with plain vision transformers. 
For non-hierarchical backbones, such as ViT, the resolution is maintained and the last layer feature map contains the richest semantic information.  Thus, our proposed method that uses the tokens to merge features of different levels got better performance. By simply changing the FPN structure with out ATM based Token merge, we improve the performance from 46.7\% to 50.6\%.
For the loss type, pixel level loss indicates the regular cross-entropy loss applied to the feature map. The dot product loss indicates the loss used in \cite{detr} and \cite{maskformer}. 
Attention mask loss means the mask supervision is directly applied to the similarity map generated by the ATM during attention calculation. We can see that the loss supervised on the attention mask further improve the result with 0.6\%. 


\begin{table}[]
\centering
\setlength{\tabcolsep}{1.5pt}
\footnotesize
\caption{Ablation results of different decoder methods with their corresponding feature merge types and loss types. ViT-Base is employed as the backbone for all the variants.}
\vspace{0.5em}
\label{tab:struct compare}

\begin{tabular}{rcccccc}
\toprule
\multicolumn{1}{c}{} & \multicolumn{2}{c}{Multi-level Features} & \multicolumn{3}{c}{Loss Types} & \multicolumn{1}{c}{} \\ 
\cmidrule(r){2-3}
\cmidrule(l){4-6}
\multicolumn{1}{c}{Decoder} & FPN & \multicolumn{1}{c}{Token Merge} & Pixel level & Dot product & Attention Mask & \multicolumn{1}{c}{mIoU (ss)} \\ 
\midrule
SETR-MLA \cite{setr}& \checkmark & \multicolumn{1}{c}{} & \checkmark &  &  & 48.2 \\
Segmenter \cite{strudel2021segmenter} &  & \multicolumn{1}{c}{} & \checkmark &  &  & 49.0 \\
MaskFormer \cite{maskformer} & \checkmark & \multicolumn{1}{c}{} &  & \checkmark &  & 46.7 \\
Ours-Variant 1 &  & \multicolumn{1}{c}{} &  &  & \checkmark & 49.6 \\
Ours-Variant 2&  & \multicolumn{1}{c}{\checkmark} &  & \checkmark &  & 50.6 \\
Ours &  & \multicolumn{1}{c}{\checkmark} &  &  & \checkmark & 51.2 \\ 
\bottomrule
\end{tabular}

\end{table}




